Automated Robot Recovery from Assumption Violations of High-Level Specifications

This paper presents a framework that enables robots to automatically recover from assumption violations of high-level specifications during task execution. In contrast to previous methods relying on user intervention to impose additional assumptions for failure recovery, our approach leverages synthesis-based repair to suggest new robot skills that, when implemented, repair the task. Our approach detects violations of environment safety assumptions during the task execution, relaxes the assumptions to admit observed environment behaviors, and acquires new robot skills for task completion. We demonstrate our approach with a Hello Robot Stretch in a factory-like scenario.

==> algorithms/compute_winning_states.tex <==
\begin{algorithm}[h]
\KwIn{Game structure $\game$ where $\obj = \bigwedge_{i=1:m} J^e_i \to \bigwedge_{j=1:n} J^s_j$} 
\KwOut{Target states $T$, Winning states $\winning$, Boolean $\textrm{repair}$ indicating if repair is needed}

$Z \coloneqq \inpstates, Z' \coloneqq \emptyset$\;
\While{$(Z' \neq Z)$}{
    $Z' \coloneqq Z$\;
    \For{$(j = 1; j \leq n; j++)$}{
        $Y \coloneqq \emptyset, Y' \coloneqq \inpstates$\;
        \While{$(Y' \neq Y)$}{
            $Y' \coloneqq Y$\;
             $\tt{start} \coloneqq J^s_j \cap \CPre(Z)$\;
            \If{\tt{start} $= \emptyset$}{
                \Return $(J^s_j, \winning, \true)$\;
            }
            $\tt{start} \coloneqq \tt{start} \cup \CPre(Y)$\;
            $Y \coloneqq \emptyset$\;
            \For{$(i=1; i\leq m; i++)$}{
                $X \coloneqq Z, X' \coloneqq \emptyset$\;
                \While{$(X' \neq X)$}{
                    $X' \coloneqq X$\;
                    $X \coloneqq \tt{start} \cup (\neg J^e_i \cap \CPre(X))$\;
                }
                $Y \coloneqq Y \cup X$\;
            }
        }
        $Z \coloneqq Y$\;
    }
}
\Return $(\true, \winning, \false)$\;

\caption{\textbf{compute\_winning\_states}}
\label{alg:compute_winning_states}
\end{algorithm}


==> algorithms/modify_postcondition_full.tex <==
\begin{algorithm*}[h]
\KwIn{$\tenv$, $\tsysnothard$, $Z$, $\inpuser$} 
\KwOut{$\tenvnew$}
\tcp{Find states that do not lead to winning states}
$\treachable = \{(\inpstateone, \outstateone, \inpstatetwo') \in \tenv \setor \exists \inpstatethree \in \inpstates, \outstatethree \in \outstates \textrm{ s.t. } (\inpstatethree, \outstatethree, \inpstateone', \outstateone') \in \tsysnothard \textrm{ and } (\inpstatethree, \outstatethree, \inpstateone') \in \tenv$\}\;\label{line:post_reachable}
$\tfullskills = \{(\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \allstates \times \allstatesprime \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tsysnothard,\ (\inpstateone, \outstateone, \inpstatetwo') \in \treachable,\ \outstateone \neq \emptyset\}$\;\label{line:post_full}
$\tnotwinningfullskills = \{(\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tfullskills \setor (\inpstatetwo, \outstatetwo) \notin Z  \textrm{ and } (\inpstateone, \outstateone) \notin Z\}$\;\label{line:post_notwinning}

\tcp{Find allowable changes}
$\tau_\textrm{cur-pres} = \{(\inpstateone, \outstateone) \in \allstates \setor (\inpstateone, \outstateone, \inpstatetwo) \in \treachable \}$\;
$\tallowablechanges = \{(\inpstateone, \outstateone, \inpstatetwo', \outstatetwo', \inpstatethree^{\dagger}) \in \allstates \times \allstatesprime \times \inpstatesdoubleprime \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tnotwinningfullskills,\ (\inpstatetwo, \inpstatethree') \in \tchangeconstraints,\ (\inpstateone, \outstateone, \inpstatethree') \in \tnotallowedrepair,\ \inpstateone \neq \inpstatethree,\ (\inpstatethree, \outstatetwo) \in Z, (\inpstateone, \outstateone, \inpstatethree', \outstatetwo') \in \tsysnothard, \textrm{ and } ((\inpstatethree, \outstateone) \notin \tau_\textrm{cur-pre} \textrm{ or } (\inpstateone, \outstateone, \inpstatethree') \in \treachable)\}$\;\label{line:post_allowablechanges}
\eIf{$\tallowablechanges \neq \emptyset$}{
$\tselectedchange = \textrm{randomlySelectOne}(\tallowablechanges)$\;\label{line:post_selectedchange}
$\tselectedchange = \{(\inpstateone, \outstateone, \inpstatetwo', \outstatetwo', \inpstatethree^{\dagger} \in \allstates \times \allstatesprime \times \inpstatesdoubleprime \setor (\inpstateonea, \outstateone, \inpstatetwoa', \outstatetwo', \inpstatethreea^{\dagger}) \in \tselectedchange, \statevar_\textrm{u} \in 2^{\inpuser}, \inpstateone = (\inpstateonea \setminus \inpuser) \cup \statevar_\textrm{u}, \inpstatetwo = (\inpstatetwoa \setminus \inpuser) \cup \statevar_\textrm{u}, \inpstatethree = (\inpstatethreea \setminus \inpuser) \cup \statevar_\textrm{u}\}$\;\label{line:post_alluservariables}
}
{\Return $\tenv$}

\tcp{Modify $\tenv$}
$\tenvadd = \{(\inpstateone, \outstateone, \inpstatethree')\in \allstates \times \inpstatesprime \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo', \inpstatethree^{\dagger}) \in \tselectedchange\}$\;\label{line:post_tenvadd}
$\tenvold = \{(\inpstateone, \outstateone, \inpstatetwo') \in \allstates \times \inpstatesprime \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo', \inpstatethree^{\dagger}) \in \tselectedchange\}$\;\label{line:post_tenvold}
$\tenvnew = (\tenv \setminus \tenvold) \cup \tenvadd$\;\label{line:post_tenvnew}

\Return $\tenvnew$
\caption{\textbf{modify\_postconditions\_full}}
\label{alg:modify_post_full}
\end{algorithm*}


==> algorithms/modify_postcondition_simple.tex <==
\begin{algorithm}[h]
\KwIn{$\tenv$, $\tsysnothard$, $Z$, $\inpuser$} 
\KwOut{$\tenvnew$}

\tcp{Find states that do not lead to winning states}
$\tfullskills = \textrm{findReachableSkills}(\tsysnothard, \tenv)$\;\label{line:simple_post_full}
$\tnotwinningfullskills = \textrm{findNotWinningSkills}(\tfullskills, Z)$\;\label{line:simple_post_notwinning}

\tcp{Find allowable changes}
$\tallowablechanges = \textrm{findAllowableChanges}(\tnotwinningfullskills,\allowbreak \tchangeconstraints,\allowbreak \tnotallowedrepair,\allowbreak \tsysnothard,\allowbreak \tenv, Z)$\;\label{line:simple_post_allowablechanges}
\eIf{$\tallowablechanges \neq \emptyset$}{
$\tselectedchange = \textrm{randomlySelectOneChange}(\tallowablechanges)$\;\label{line:simple_post_selectedchange}
$\tselectedchange = \textrm{removeDependenceOnUserPropositions}(\allowbreak\tselectedchange,\allowbreak \inpuser)$\;\label{line:simple_post_alluservariables}
}
{\Return $\tenv$}

\tcp{Modify $\tenv$}
$\tenvadd = \textrm{findEnvTransitionsToAdd}(\tselectedchange)$\;\label{line:simple_post_tenvadd}
$\tenvold = \textrm{findEnvTransitionsToRemove}(\tselectedchange)$\;\label{line:simple_post_tenvold}
$\tenvnew = (\tenv \setminus \tenvold) \cup \tenvadd$\;\label{line:simple_post_tenvnew}

\Return $\tenvnew$
\caption{\textbf{modify\_postconditions\_simple}}
\label{alg:modify_post_simple}
\end{algorithm}


==> algorithms/modify_precondition_full.tex <==

\begin{algorithm*}[h]

\KwIn{$\tenv$, $\tenvhard$, $\tsysnothard$, $\tsyshard$, $\winning$, $\inpuser$}
\KwOut{$\tenvnew$, $\tsysnewmutable$}
\BlankLine

\tcp{Find states where the system is guaranteed to reach $\winning$ for any environment choice}
$\tsyscanwin = \{(\inpstateone, \outstateone, \inpstatetwo')\in \allstates \times \inpstatesprime \setor \exists \inpstateone, \inpstatetwo \in \inpstates, \outstateone, \outstatetwo \in \outstates \textrm{ s.t. } (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tsysnothard \textrm{ and } (\inpstatetwo, \outstatetwo) \in Z\}$\;\label{line:pre_syscanwin}

$\tsysalwayswins = \{(\inpstateone, \outstate) \in \allstates \setor \forall \inpstatetwo \in 2^{\inpsyms} \textrm{ s.t. } (\inpstateone, \outstate, \inpstatetwo') \in \tenv \rightarrow (\inpstateone, \outstate, \inpstatetwo') \in \tsyscanwin, \outstate \neq \emptyset\}$\;\label{line:pre_sysalwayswins}

$\treachable = \{(\inpstateone, \outstateone, \inpstatetwo') \in \tenv \setor \exists \inpstatethree \in \inpstates, \outstatethree \in \outstates \textrm{ s.t. } (\inpstatethree, \outstatethree, \inpstateone', \outstateone') \in \tsysnothard \textrm{ and } (\inpstatethree, \outstatethree, \inpstateone') \in \tenv$\}\;\label{line:pre_reachable}

$\tcanwinandencoded = \{ (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \allstates \times  \allstatesprime \setor (\inpstateone, \outstateone) \in \tsysalwayswins,\ (\inpstatetwo, \outstatetwo) \in Z,\ (\inpstateone, \outstateone, \inpstatetwo') \in \treachable, (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tsysnothard\}$\;\label{line:pre_canwinandencoded}

\tcp{Find allowed changes to preconditions}
$\tau_\textrm{skills-changing} = \{\outstateone \in \outstates \setor \exists \inpstateone, \inpstatetwo \in \inpstates, \outstatetwo \in \outstates \textrm{ s.t. } (\inpstateone, \outstateone, \inpstateone', \inpstatetwo') \in \tcanwinandencoded\} $\;\label{line:pre_skillschanging}
$\tpreskills=\{(\inpstateone, \outstate) \in \allstates \setor \exists \inpstatetwo \in \inpstates \textrm{ s.t. } (\inpstateone, \outstate, \inpstatetwo) \in \treachable \textrm{ and } \outstate \in \tau_\textrm{skills-changing}\}$\;\label{line:pre_preskills}
$\tfinalpost=\{(\outstate, \inpstateone') \in \outstates \times \inpstatesprime \setor \exists \inpstatetwo \in \inpstates \textrm{ and } \nexists \inpstatethree \in \inpstates \textrm{ s.t. } (\inpstatetwo, \outstate, \inpstateone) \in \treachable \textrm{ and } (\inpstateone, \outstate, \inpstatethree) \in \treachable\}$\;\label{line:pre_finalpost}
$\tallowablechanges = \{ (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo', \inpstatethree^{\dagger}) \in \allstates \times \allstatesprime \times \inpstatesdoubleprime \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tcanwinandencoded,\ (\inpstateone, \inpstatethree') \in \tchangeconstraints,\ (\inpstatethree, \outstateone, \inpstatetwo') \in \tnotallowedrepair,\ (\inpstatethree, \outstateone) \notin \tpreskills,\ (\inpstatethree, \outstateone, \inpstatetwo', \outstatetwo') \in \tsyshard,\ (\inpstatethree, \outstateone, \inpstatetwo', \outstatetwo') \notin \tcanwinandencoded,\ \inpstatethree \neq \inpstatetwo,\ (\outstate, \inpstatethree') \notin \tfinalpost\}$\;\label{line:pre_allowablechanges}

\tcp{Randomly select one possible change to add}
\eIf{$\tallowablechanges \neq \emptyset$}{
$\tselectedchange = \textrm{randomlySelectOne}(\tallowablechanges)$\label{line:pre_selectedchange}\;
$\tselectedchange = \{(\inpstateone, \outstateone, \inpstatetwo', \outstatetwo', \inpstatethree^{\dagger})\in \allstates \times \allstatesprime \times \inpstatesdoubleprime \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tsysnothard \textrm{ and } \exists \outstatethree \in \outstates \textrm{ s.t. } (\inpstateone, \outstateone, \inpstatetwo', \outstatethree', \inpstatethree^{\dagger}) \in \tselectedchange\}$\;\label{line:pre_selectadditionalchanges}
$\tselectedchange = \{(\inpstateone, \outstateone, \inpstatetwo', \outstatetwo', \inpstatethree^{\dagger}) \in \allstates \times \allstatesprime \times \inpstatesdoubleprime \setor (\inpstateonea, \outstateone, \inpstatetwoa', \outstatetwo, \inpstatethreea^{\dagger}) \in \tselectedchange, \statevar_\textrm{u} \in 2^{\inpuser}, \inpstateone = (\inpstateonea \setminus \inpuser) \cup \statevar_\textrm{u}, \inpstatetwo = (\inpstatetwoa \setminus \inpuser) \cup \statevar_\textrm{u}, \inpstatethree = (\inpstatethreea \setminus \inpuser) \cup \statevar_\textrm{u}\}$\;\label{line:pre_alluservariables}
}
{
\Return $\tenv$, $\tsysnothard$\
}
$\tnewfullskill = \{(\inpstatethree, \outstateone, \inpstatetwo', \outstatetwo') \in \allstates \times \allstatesprime \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo', \inpstatethree^{\dagger}) \in \tselectedchange \}$\;\label{line:pre_newfullskill}

\tcp{Add transitions to $\tsysnothard$}

$\toldfullskill = \{(\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \allstates \times \allstatesprime \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo', \inpstatethree^{\dagger}) \in \tselectedchange \}$\;\label{line:pre_oldfullskill}

$\toldprepreconditions = \{\inpstateone, \outstateone) \in \allstates \setor (\inpstatetwo, \outstatetwo, \inpstatethree, \outstatethree) \in \toldfullskill \textrm{ and } (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tsysnothard\}$\;\label{line:pre_oldprepreconditions}
$\tnewpreprecondition = \{(\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \allstates \times \allstatesprime \setor (\inpstateone, \outstateone) \in \toldprepreconditions \textrm{ and } (\inpstatetwo, \outstatetwo, \inpstatethree, \outstatethree) \in \tnewfullskill\}$\;\label{line:pre_newprepreconditions}

\tcp{Determine if this is the initial precondition}
\If{$\{(\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \allstates \times \allstatesprime \setor \forall \outstateone \in \outstates, (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tnewpreprecondition\} == \tnewpreprecondition$}{\label{line:pre_modinitprecheck} 
$\tau_\textrm{only-input-props} = \{\inpstatetwo \in \inpstate \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tnewpreprecondition\}$\;
$\tau_\textrm{diff-skills-with-same-pre} = \{(\inpstateone, \inpstatetwo, \outstatetwo) \in \inpstates \times \allstates \setor \forall \outstateone \in \outstate, (\inpstateone, \outstateone, \inpstatetwo, \outstatetwo) \in \tsysnothard \textrm{ and } \inpstatetwo \in \tau_\textrm{only-input-props}\}$\;\label{line:pre_allskillscanbeapplied}
$\tau_\textrm{remove} = \{(\inpstateone, \outstateone, \inpstatetwo') \in \allstates \times \inpstatesprime \setor \exists \outstatetwo \in \outstates \textrm{ s.t. } (\inpstateone, \outstateone, \inpstatetwo, \outstatetwo) \in \tsysnothard \textrm{ and } (\inpstateone, \inpstatetwo, \outstatetwo) \notin \tau_\textrm{diff-skills-with-same-pre} \textrm{ and } \inpstatetwo \in \tau_\textrm{only-input-props}\}$\;\label{line:pre_remove}
$\tnewpreprecondition = \{(\inpstateone, \outstateone, \inpstatetwo, \outstatetwo) \in \tnewpreprecondition \setor (\inpstateone, \outstateone, \inpstatetwo') \notin \tau_\textrm{remove}\}$\;\label{line:pre_newprepreconditions2}
}
$\tsysnewmutable = \tsysnothard \cup \tnewpreprecondition \cup \tnewfullskill$\;\label{line:pre_sysnothardnew}

\tcp{Add transitions to $\tenv$}

$\tenvpreold = \{(\inpstateone, \outstateone) \in \allstates\setor (\inpstateone, \outstateone, \inpstatetwo') \in\treachable \textrm{ and } (\inpstatetwo, \outstateone, \inpstatethree', \outstatethree') \in \toldfullskill\}$\;\label{line:pre_envpreold}
$\tenvprenew = \{(\inpstateone, \outstateone, \inpstatetwo') \in \allstates \times \inpstatesprime \setor (\inpstateone, \outstateone) \in \tenvpreold,\ (\inpstatetwo, \outstateone, \inpstatethree', \outstatethree') \in \tnewfullskill\}$\;\label{line:pre_envprenew}
$\tenvnewfullskill = \{(\inpstateone, \outstateone, \inpstatetwo') \in \allstates \times \inpstatesprime \setor (\inpstateone, \outstateone, \inpstatetwo', \outstatetwo') \in \tnewfullskill\}$\;\label{line:pre_envnewfullskill}
$\tenvnew = (\{(\inpstateone, \outstateone, \inpstatetwo') \in \tenv \setor \nexists \inpstatethree, \outstatethree \textrm{ s.t. } (\inpstateone, \outstateone, \inpstatethree', \outstatethree') \in \tnewfullskill\} \cup \tenvnewfullskill \cup \tenvprenew) \cap \tenvhard$\;\label{line:pre_envnew2}
\Return $\tenvnew$, $\tsysnewmutable$
\caption{\textbf{modify\_preconditions\_full}}
\label{alg:modify_pre_full}
\end{algorithm*}

==> algorithms/modify_precondition_simple.tex <==
\begin{algorithm*}[h]
\KwIn{$\tenv$, $\tenvhard$, $\tsysnothard$, $\tsyshard$, $\winning$, $\inpuser$}
\KwOut{$\tenvnew$, $\tsysnewmutable$}
\BlankLine
\tcp{States where the system is guaranteed to reach $Z$ for any environment choice}

$\tcanwinandencoded = \textrm{systemAlwaysWinsAndSkillsAreReachable}(\tsysnothard, \tenv, Z)$\;\label{line:simple_pre_canwinandencoded}

\tcp{Find allowed changes to preconditions}
$\tallowablechanges = \textrm{findAllowableChanges}(\tcanwinandencoded, \tchangeconstraints, \tnotallowedrepair, \tsyshard, \tenv)$\;\label{line:simple_pre_allowablechanges}

\tcp{Randomly select the possible change to add}
\eIf{$\tallowablechanges \neq \emptyset$}{
$\tselectedchange = \textrm{randomlySelectChange}(\tallowablechanges, \tsysnothard)$\label{line:simple_pre_selectedchange}\;
$\tselectedchange = \textrm{removeDependenceOnUserPropositions}(\tselectedchange, \inpuser)$\;\label{line:simple_line_pre_alluservariables}
}
{
\Return $\tenv$, $\tsysnothard$\;
}
$\tnewfullskill = \textrm{replacePreconditions}(\tselectedchange)$\;\label{line:simple_pre_newfullskill}

\tcp{Add transitions to $\tsysnothard$}
$\tnewpreprecondition = \textrm{addPrePrecondition}(\tselectedchange, \tsysnothard)$\;\label{line:simple_pre_newprepreconditions}

\tcp{Determine if this is the initial precondition}
\If{$\textrm{isInitialPrecondition}(\tnewpreprecondition)$}{\label{line:simple_pre_modinitprecheck}
$\tnewpreprecondition =\textrm{disallowExecutionFromOtherIntermediateStates}(\tsysnothard, \tnewpreprecondition)$\;\label{line:simple_pre_newprepreconditions2}
}
$\tsysnewmutable = \tsysnothard \cup \tnewpreprecondition \cup \tnewfullskill$\;\label{line:simple_pre_sysnothardnew}

\tcp{Add transitions to $\tenv$}

$\tenvnew = \textrm{createNewEnvTransition}(\tenv, \tenvhard, \tnewfullskill, \tselectedchange, \tsysnothard)$\;\label{line:simple_pre_envnew2}
\Return $\tenvnew$, $\tsysnewmutable$
\caption{\textbf{modify\_preconditions\_simple}}
\label{alg:modify_pre_simple}
\end{algorithm*}

==> algorithms/perform_repair.tex <==
\begin{algorithm}[h]
\KwIn{Game structure $\game$, 
        Target states $T$, 
        Winning states $\winning$, 
        Boolean $\tt{cover}$ ($\true$ if all of $T$ must become winning), 
        Dictionary $\tt{opts}$ which includes 
        a Boolean $\tt{post\_first}$ indicating whether to perform modify-postcondiion first and 
        a Boolean $\tt{one\_repair}$ indicating whether to return with one repair only
        % Hard system transitions $\tsyshard$
        }
\KwOut{A modified game structure $\gamemod$}

$\tenvmod \coloneqq \tenv, \tsysmod \coloneqq \tsys$\;
\While{$\true$}{
    $\winning' \coloneqq \emptyset$\;
    \While{$\winning' \neq \winning$}{
        $\winning' \coloneqq \winning$\;
        $\winning \coloneqq \winning \cup \CPre(\winning)$\;
    }
    $\tt{overlap} \coloneqq T \cap \CPre(\winning)$\;
    \If{$\tt{overlap} = T$ or ($\neg \tt{cover}$ and $\tt{overlap} \neq \emptyset$) }{
        break\;
    }
    \eIf{$\tt{opts[post\_first]}$}{
        $\tenvtmp \coloneqq \mathbf{modify\_postconditions}(\gamemod, \winning)$\;
        $\tsystmp \coloneqq \tsysmod$\;
        \eIf{$\tenvtmp = \tenvmod$}{
            $\tsystmp \coloneqq \mathbf{modify\_preconditions}(\gamemod, \winning)$\;
        }{
            $\tt{opts[post\_first]} \coloneqq \false$\;
        } 
    }{
        $\tsystmp \coloneqq \mathbf{modify\_preconditions}(\gamemod, \winning)$\;
        $\tenvtmp \coloneqq \tenvmod$\;
        \eIf{$\tsystmp = \tsysmod$}{
            $\tenvtmp \coloneqq \mathbf{modify\_postconditions}(\gamemod, \winning)$\;
        }{
            $\tt{opts[post\_first]} \coloneqq \true$\;
        }
    }
    \eIf{$\tenvtmp = \tenvmod$ $\tt{and}$ $\tsystmp = \tsysmod$}{
        \Return \textbf{no repair}\;
    }{
        \If{$\tt{opts[one\_repair]}$}{
            break\;
        }
    }
    
    
    
    
}
\Return $\tenvmod, \tsysmod$\;

\caption{\textbf{perform\_repair}}
\label{alg:perform_repair}
\end{algorithm}

==> algorithms/skill_reduction.tex <==
\begin{algorithm}[t]
\KwIn{Original spec $\oldspec$, skills $\outnew$} 
\KwOut{A minimal subset of $\outnew$}
% $\outnew' \coloneqq \emptyset$\;
    \For{$y \in \outnew$}{
        $\outnew \coloneqq \outnew\setminus y$\; \label{alg:sr_setminus}
        $\newspec \coloneqq \textrm{addSkillsToSpec}(\outnew, \oldspec)$\; \label{alg:sr_addskill}
        $\strategy \coloneqq \textrm{synthesize}(\newspec)$\; \label{alg:sr_synthesize}
        \If{$\newspec$ is unrealizable ($\strategy$ is None)}{
            $\outnew \coloneqq \outnew \cup \{y\}$\; \label{alg:sr_setadd}
            % $\outnew' \coloneqq \outnew' \cup \{y\}$\; \label{alg:sr_setadd2}
        }
    }
    {\Return $\outnew$}
\caption{\textbf{skill\_reduction}}
\label{alg:skill_reduction}
\end{algorithm}

==> algorithms/symbolic_repair.tex <==
\begin{algorithm}[h]
\KwIn{Specification $\varphi$, 
        A dictionary of hyperparameters \texttt{opts}
        }
\KwOut{A set of suggested skills $\outsuggest$}

$\game \coloneqq \mathbf{spec\_to\_game}(\varphi)$\;
$\gamemod \coloneqq \game, \initstates \coloneqq \game.\tt{get\_init}()$\;
$\tt{repair} \coloneqq \true$\;
\While{$\tt{repair}$}{
    \tcp{Check overlap of liveness goals}
    $T, \winning, \tt{repair} \coloneqq \mathbf{compute\_winning\_states(\gamemod)}$\;
    \If{$\tt{repair}$}{
        $\gamemod \coloneqq \mathbf{perform\_repair}(\gamemod, T, \winning, \false, \tt{opts})$\;
    }
}
\While{$\initstates \not\subseteq \winning$}{
    \tcp{Check coverage of initial states}
    $\gamemod \coloneqq \mathbf{perform\_repair}(\gamemod, \initstates, \winning, \true, \tt{opts})$\;
    $T, \winning, \tt{repair} \coloneqq \mathbf{compute\_winning\_states(\gamemod)}$\;
}
$\cA \coloneqq \mathbf{synthesize\_and\_determinize}(\gamemod, \winning)$\;
$\outsuggest \coloneqq \mathbf{extract\_suggestions}(\cA, \game)$\;
\Return $\outsuggest$\;


\caption{\textbf{synthesis\_based\_repair}}
\label{alg:symbolic_repair}
\end{algorithm}

==> figures/compiler_workflow.tex <==
% \begin{figure}[t]
    \centering
    \includegraphics
    [width=0.45\textwidth]{figures/compiler_workflow.png}
    \caption{Workflow of the violation detection procedure.}
    \label{fig:compiler}
\end{figure}

==> figures/factory_workspace_full.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.486\textwidth]{figures/workspace_objects.png}
    \caption{Stretch physical experiment in the lab. 
    (A) The physical workspace.
    (B) The initial positions of the objects in the workspace.}
    \label{fig:factory_workspace_full}
\end{figure}

==> figures/restaurant_example_one_workspace.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/restaurant_example_one_workspace.png}
    \caption{Workspace for Example 1}
    \label{fig:restaurant_example_one_workspace}
\end{figure}

==> sections/7.2_optimization.tex <==
\subsection{Optimization}
% Reduce the size of the set of suggested skills
We optimize the repair algorithm's output by reducing the size of the suggested skills while ensuring that the new specification remains realizable.  
Since the repair algorithm in~\cite{pacheck2020finding} does not consider the minimality of the suggested skills, 
the suggested skills may contain redundant skills. 
% Add a practical example to describe the percentage of the useless suggested skills (?)
We propose a skill-reduction procedure to remove the unnecessary suggested skills. 
Given an unrealizable specification and a set of suggested skills from the repair algorithm, 
the skill-reduction procedure finds a subset of the suggested skills that can make the original specification realizable. 

Algorithm~\ref{alg:skill_reduction} describes the skill-reduction procedure. 
For each suggested skill, the procedure removes the skill from the set of suggested skills (Line \ref{alg:sr_setminus}) 
and adds the rest of the suggested skills to the original specification represented by the ASTs in the compiler (Line \ref{alg:sr_addskill})). 
We then generate the new specification from the modified ASTs and use Slugs to check for the realizability of the specification (Line \ref{alg:sr_synthesize}). 
If the result is realizable, then the removed skill is not required to make the specification realizable, so we remove the skill permanently. 
Otherwise, the removed skill is necessary, so we add the skill back to the set of suggested skills and to a set of necessary skills (Line \ref{alg:sr_setadd}, \ref{alg:sr_setadd2}). 
Lastly, the procedure adds the necessary skills to the original specification.  

\input{algorithms/skill_reduction}

We note that the skill-reduction procedure does not guarantee finding the \emph{minimum} subset of necessary suggested skills. 
There may exist another subset of the suggested skills with fewer skills that can make the specification realizable. 
Instead, the procedure finds a \emph{minimal} subset of necessary suggested skills. 
Removing any skill from the subset of skills results in the unrealizability of the specification, 
because otherwise the skill will be removed by the procedure. 
Note that we can find the minimum subset of necessary skills by calling Algorithm~\ref{alg:skill_reduction} for each permutation of the suggested skills and returning the smallest subset of skills. 
However, the time complexity of this approach is higher because  
for $n$ suggested skills, it calls the synthesis algorithm $n!$ times, while Algorithm~\ref{alg:skill_reduction} calls the synthesis algorithm $n$ times, 
and the time complexity of the synthesis algorithm is 
singly exponential in the size of the specification. 
Therefore, we prioritize reducing the number of calls of the synthesis algorithm and  
only use Algorithm~\ref{alg:skill_reduction} to perform the optimization in practice. 


==> sections/7.3_physical_implementation.tex <==
\subsection{Implementation}
% Symbolic repair vs physical implementability tradeoff
% Skill implementation

Our framework provides the physical implementation of the new skills. 
We are given a new skill $y \in \outnew$ and its symbolic representation in the format of a list of intermediate states. 
The list of intermediate states infers a list of waypoints of the skill. 

% Given a new skill y_{\textrm{new}} \in \outnew

\qm{\todo we only have skill implementation on one controller (base controller), if there are multiple controllers, the new skill should be implemented by the same controller as the old skill, and the intermediate states infer the waypoints of the skill. We also need to implement and discuss the tradeoff of the physical implementability checking}


==> sections/sltl.tex <==
We define \gls{sltl}, a subclass of \gls{ltl} in which the only temporal operator is the next operator. 
We define the syntax of \gls{sltl} using the following grammar: 
\begin{align*}
    \spec \qquad \coloneqq \qquad   &   t \MID{} t \land t \tag{formulas}\\
    t \qquad \coloneqq \qquad       &   v \MID{} \neg v \tag{terms}\\
    v \qquad \coloneqq \qquad       &   \pi \MID{} \bigcirc \pi \tag{variables}
\end{align*}
We can derive other Boolean operators from the grammar. 

We define the semantics of \gls{sltl} over $2^{\vars \cup \bigcirc \vars}$ and 
denote by $\denote{\psi}$ the set of subsets of $\vars \cup \bigcirc \vars$ satisfying an \gls{sltl} formula $\psi$. 
A subset $S \subseteq \vars \cup \bigcirc \vars$ is in $\denote{\psi}$ iff 
for any variable $v \in \vars \cup \bigcirc \vars$ that appears in $\psi$ as a term, $v \in S$ and for any $v$ whose negation appears as a term, $v \not\in S$. 
% A variable $v \in \vars \cup \bigcirc \vars$ is in $\denote{\psi}$ if $v$  appears 

% Formally, the semantics of a \gls{sltl} formula $\psi$ is defined as 
% $\denote{\psi} \coloneqq \{v \in \vars \cup \bigcirc \vars \mid v \text{appears }\}$

==> sections/todo.tex <==
\section{Todo}
\begin{enumerate}
    \item Physical implementability checking for repair
    \begin{enumerate}
        \item Nine square implementability checking
        \item Tradeoff between purely symbolic repair and with physical implementability checking added. Why not allowing valid transitions only in the safety constraints?
    \end{enumerate}
    \item Demonstration
    \begin{enumerate}
        \item \emph{Scenario briefing}. 
        The robot operates in a restaurant setting as a waiter. 
        The workspace consists of three tables, representing a kitchen, a dining table, and a sink, respectively. 
        The objects of interest include a cup, two plates, two blocks, the robot base, and the robot end-effector (ee). 
        Initially, one plate, the cup, and the blocks are on the kitchen table, and the other plate is on the sink table. 
        The cup is on top of the plate. 
        The customer has three buttons to request appetizers, drinks, and main dishes. 
        Once a button is pushed, the robot delivers the corresponding object to the dining table. 
        If a plate is empty (the block is gone) on the dining table, the robot should deliver the empty plate to the sink. 
        There cannot be two plates in the same region. 
        
        The customer first pushes the appetizer button. 
        The robot needs to first move the cup to another region, then stack the appetizer block onto the plate, and finally move the plate to the central region of the dining table.
        The appetizer block is blocked by the main dish block, so the robot needs to first move the main dish block away, and then move the appetizer block
        
        The customer next pushes the drink button while eating the appetizer. 
        The robot goes back to pick up the cup and delivers the cup to the left region of the dining table. 
        By then, the appetizer plate is empty, so the robot delivers it to the sink, but before that, it moves the plate from the sink to the kitchen. 
        During the pickup, the customer accidentally pushes the plate so the pickup is unsuccessful. 
        The recovery process learns a new skill to pick up the plate. 

        Lastly, the customer pushes the main dish button. 
        The robot stacks the main dish onto the plate on the kitchen table and then delivers it to the central region of the dining table. 
        After the customer finishes the meal, the customer accidentally puts the plate onto another region, thus violating the assumption. 
        The robot moves the plate to the sink after the customer finishes, before moving the plate out of the sink. 

        
        \item Abstraction
        \begin{enumerate}
            \item Workspace (Figure~\ref{fig:workspace})
            \begin{enumerate}
                \item Ground: $x_0 \dots x_2$, $y_0 \dots y_2$
                \item Kitchen: $k_0 \dots k_4$
                \item Sink: $s_0, s_1$
                \item Dining table: $t_0 \dots t_2$
            \end{enumerate}
            \item Objects
            \begin{enumerate}
                \item Robot base: base
                \item Robot gripper: ee
                \item Plates: $\textrm{plate}_0, \textrm{plate}_1$
                \item Cup: cup
                \item Blocks: $b_0, b_1$
                \item Obstacle: cone
                \item Manipulation obstacle
            \end{enumerate}
            \item Inputs $\inp$
        \end{enumerate}

        \item Skills
        \begin{enumerate}
            \item skill0 (base): $x_1 \land y_2 \to x_1 \land y_1 \to x_1 \land y_0$
        \end{enumerate}
        
        \item Potential Violations 
        \begin{enumerate}
            \item Unexpected base obstacle location
            \item Unexpected manipulation obstacle location
            \item Unexpected plates/cup/blocks location
            \item Unexpected block-plate relation
            \item Unexpected base/ee location (low-level skill failure)
            \item Unexpected indoor environment/topology, e.g. the sink becomes unreachable (hard to repair)
            \item Unexpected ee-manipulation object relation (low-level skill failure)
        \end{enumerate}
        \item Specification
        \item Reactivity discussion
    \end{enumerate}
\end{enumerate}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/workspace.jpeg}
    \caption{Workspace}
    \label{fig:workspace}
\end{figure}
